PEMA: An Offsite-Tunable Plug-in External Memory Adaptation for Language Models

Pre-trained language models (PLMs) show impressive performance in various downstream NLP tasks. However, pre-training large language models demands substantial memory and training compute. Furthermore, due to the substantial resources required, many PLM weights are confidential. Consequently, users are compelled to share their data with model owners for fine-tuning specific tasks. To overcome the limitations, we introduce Plug-in External Memory Adaptation (PEMA), a Parameter-Efficient Fine-Tuning (PEFT) method, enabling PLM fine-tuning without requiring access to all the weights. PEMA integrates with context representations from test data during inference to perform downstream tasks. It uses external memory to store PLM-generated context representations mapped with target tokens. Our method utilizes weight matrices of LoRA-like bottlenecked adapter in the PLM's final layer to enhance efficiency. Our approach also includes Gradual Unrolling, a novel interpolation strategy to improve generation quality. We validate PEMA's effectiveness through experiments on syntactic and real datasets for machine translation and style transfer. Our findings show that PEMA outperforms other PEFT approaches in memory and latency efficiency for training, and also excels in maintaining sentence meaning and generating appropriate language and styles.

==> abstract.tex <==
\begin{abstract}
Pre-trained language models (PLMs) have demonstrated impressive performance across various downstream NLP tasks. 
Nevertheless, the resource requirements of pre-training large language models in terms of memory and training compute pose significant challenges. 
Furthermore, due to the substantial resources required, many PLM weights are confidential. 
Consequently, users are compelled to share their data with model owners for fine-tuning specific tasks.
To overcome the limitations, we introduce Plug-in External Memory Adaptation (\sys), a Parameter-Efficient Fine-Tuning (PEFT) approach designed for fine-tuning PLMs without the need for all weights.  
\sys can be integrated into the context representation of test data during inference to execute downstream tasks.
It leverages an external memory to store context representations generated by a PLM, mapped with the desired target token. 
Our method entails training LoRA-based weight matrices within the final layer of the PLM for enhanced efficiency. 
The probability is then interpolated with the next-token distribution from the PLM to perform downstream tasks.
To improve the generation quality, we propose a novel interpolation strategy named Gradual Unrolling.
To demonstrate the effectiveness of our proposed method, we conduct experiments to demonstrate the efficacy of \sys with a syntactic dataset and assess its performance on machine translation and style transfer tasks using real datasets.
\sys outperforms other PEFT methods in terms of memory and latency efficiency for training and inference. Furthermore, it outperforms other baselines in preserving the meaning of sentences while generating appropriate language and styles.
\end{abstract}



==> discussion.tex <==
\section{Discussions}
In this section, we discuss the XXX and limitations of \sys.

\subsection{External Memory Size}
One of the key points to consider in our approach is the size of the external memory. As the size of the external memory increases, it may lead to higher computational and memory requirements. Therefore, finding an optimal balance between memory size and performance is crucial. While a larger memory can potentially capture more diverse hidden context representations, it also introduces practical limitations, particularly for resource-constrained systems.
% 할 것이라면 Table 12에 있는 WMT22에서 length를 100만, 200만, 300만, 500만, 1000만, 전부 (random selction)해서 성능 그래프로 보여주고 그걸 appendix로 넘기기
% Appendix에 section 하나에 이거 얘기

\subsection{Performance depends on pre-trained Models and Tasks}
The effectiveness of our \sys approach is subject to the specific pre-trained language model used and the nature of the tasks it is applied. While \sys has shown promising results in our experiments, its performance might vary depending on different language models' characteristics and the complexity of downstream tasks.
% Table 1 보면서 추가 얘기를 해도 되지만 사실 그럴거면 기존에 results section에서 얘기를 해야죠.? 거기서 상세하게 얘기하기.

\subsection{Human-Defined Hyperparameters}
The hyperparameters, lambda ($\lambda$), and kappa ($\kappa$) are manually set in our approach. This human-defined setting introduces subjectivity in the fine-tuning process. The selection of these hyperparameters can significantly impact the performance of \sys. Further research is needed to explore automated methods or adaptive strategies for setting these hyperparameters to optimize the model's performance.
% Ablastion study에서 이미 얘기를 한 것이고... 이런게 한계라는 것을 알고 싶기 보다는 lambda와 kappa의 의미를 알려주는 것이 좋다. => ablation study에서 얘기를 해야하는 것. 거기서 상세하게 얘기하기.

\subsection{Generated Can Be Shorter Than the Label}
One limitation of our approach is related to situations where the pre-trained model-generated words are shorter than the label words provided. This can lead to challenges in creating the external memory, as the mapping between the hidden context representations and label words may not be straightforward. Exploring techniques to address this limitation and handling varying word lengths could enhance the adaptability of our \sys approach.


==> tbls/ablation_gsm8k.tex <==
Applied Technique     & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} & \multicolumn{1}{l}{FI} \\
\midrule
OPT-IML-30B (OPT)                            &         &        &          &     \\
OPT+Word Prediction Decoder ($B_{pd}$)       &         &        &          &     \\
OPT+PD+Graudal Unrolling (GU)                &         &        &          &     \\
OPT+GU+PD+Reconstruction Decoder ($B_{rct}$) &         &        &          &     \\
\bottomrule

==> tbls/ablation_gyafc.tex <==
Applied Technique & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} & \multicolumn{1}{l}{FormImp\%} \\
\midrule
WMT22 (EN$\rightarrow$DE) \\
\midrule
OPT-IML-MAX-30B (OPT)& 18.22& \underline{45.81} & 77.41 & \\
OPT+Word Prediction Decoder ($B_{pd}$) & 18.74& 48.05 & 77.76 & \\
OPT+$B_{pd}$+Graudal Unrolling ($GU$)& \underline{19.17}& 48.60 & \underline{78.57} & \\
OPT+$GU$+$B_{pd}$+Reconstruction Decoder ($B_{rct}$) & \textbf{19.22}&\textbf{46.62} & \textbf{79.21} & \\
\midrule
GYAFC (Family \& Relationships) \\
\midrule
OPT-IML-MAX-30B (OPT)& 60.41& 20.04 & & 29.33 \\
OPT+Word Prediction Decoder ($B_{pd}$) & 70.00& 20.38 & & 47.38 \\
OPT+$B_{pd}$+Graudal Unrolling ($GU$)& \underline{70.29}& \textbf{16.95} &  & \underline{51.24} \\
OPT+$GU$+$B_{pd}$+Reconstruction Decoder ($B_{rct}$) & \textbf{70.84} & 22.04 &  & \textbf{52.35}\\
\midrule
GYAFC (Entertainment \& Music) \\
\midrule
OPT-IML-MAX-30B (OPT)& 57.60& \textbf{21.97} &  & 23.88\\
OPT+Word Prediction Decoder ($B_{pd}$) & 64.37& 26.76 &  & 38.80\\
OPT+$B_{pd}$+Graudal Unrolling ($GU$)& \underline{64.82}& 25.62 & & \underline{42.61}\\
OPT+$GU$+$B_{pd}$+Reconstruction Decoder ($B_{rct}$) & \textbf{65.43} & \underline{25.53}&  & \textbf{44.63} \\
\bottomrule

==> tbls/ablation_wmt22.tex <==
Applied Technique & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} & \multicolumn{1}{l}{-} \\
\midrule
OPT-IML-30B (OPT)& 18.22& \underline{45.81} & 77.41 & \\
OPT+Word Prediction Decoder ($B_{pd}$) & 18.74& 48.05 & 77.76 & \\
OPT+PD+Graudal Unrolling (GU)& \underline{19.17}& 48.60 & \underline{79.12} & \\
OPT+GU+PD+Reconstruction Decoder ($B_{rct}$) & \textbf{19.22}&\textbf{46.62} & \textbf{79.21} & \\
\bottomrule

==> tbls/bad_output_low_ppl.tex <==

% bleu score 추가해야 low bleu low perplexity 얘기가 가능하다 업데이트
\sys & \\
Generated Sentences & \multicolumn{1}{c}{PPL} \\
\midrule
The Who (I think) and limp bizkit is all   I know. & 206.74 \\
\midrule
Yes, I would. & 31.50 \\
\midrule
My grandmother is a great cane kicker. & 219.62 \\
\midrule
Your mother is so stupid, she thought a   lawsuit was something you wear to court. & 47.54 \\
\midrule
I totally love them they are so hor who   else out there are dawgs that love blink 182. & 187.69 \\
\midrule
Duran, Madonna, Exile and How Could I   Forget... Air Supply!!. & 345.69 \\
\midrule
LoRA & \\
Generated Sentences & \multicolumn{1}{c}{PPL} \\
\midrule
The Who is a rock band from the United   Kingdom.  They are known for their rock   music. They are also known for their   punk rock music.  & \\
They are also known   for their heavy metal music. They are   also known for their electronic music.    They are also known for ... & 1.78 \\
\midrule
Yes, I would. I would marry Keith Urban.   He is sexy. He is a great singer. He is a great actor. He is a great   musician. He is a great father. & \\
He is a great husband. He is a great   father-in-law. He is a great husband. He is a great father. He is a great husband ...& 1.73 \\
\midrule
My grandmother is a very good cane. It is   very effective. It is very strong. It is very light. It is very flexible. It   is very strong. & \\
It is very light. It is very flexible. It is very strong. It   is very light. It is very flexible. It is very strong ...& 1.56 \\
\midrule
Yo mama's so stupid, she thought a   lawsuit was something you wear to court. The correct sentence is: Yo mama's   so stupid, she thought a lawsuit was & \\
 something you wear to court. The   sentence is formal because it is a sentence that is being used to describe. It ... & 2.35 \\
\midrule
I totally love them they are so hor who   else out there are dawgs that love blink  182??????????????????????????????????????????????????????& \\
???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????? ... & 1.80 \\
\midrule
Duran, Madonna, One Woman Band, Exile and   How Could I Forget, Air Supply, The Who, The Beatles, The Rolling Stones, The   Who, The Beatles, & \\
The Rolling Stones, The Who, The Beatles, The Rolling   Stones, The Who, The Beatles, The Rolling Stones, The Who, The Bea ... & 1.95 \\
\bottomrule



==> tbls/common_hallucinations.tex <==
Model & Common hallucination patterns \\
\midrule
OPT & I'm not sure … \\
 & I 50\% ... \\
 & Convert the following informal   sentence … \\
 & Translate this from English to   German: … \\
 & I. … \\
 & ….. … \\
\midrule
LLaMA & Informal: … \\
 & \#\#\# … \\
 & Comment: … \\
 & \textbackslash{}\textbackslash{}[ … \\
 & \textbackslash{}begin ... \\
 & Answer: … \\
\bottomrule


==> tbls/comparison_with_lora_same_parameters.tex <==
WMT22 (EN$\rightarrow$DE)& \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} \\
\midrule
OPT-IML-MAX-30B (LoRA) & 16.03& \textbf{46.97}& 74.65 \\
OPT-IML-MAX-30B (PEMA w/o rct) & \textbf{19.17}& 48.60 & \textbf{79.12} \\
\midrule
GYAFC (Family \& Relationships)& \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{FormImp} \\
\midrule
OPT-IML-MAX-30B (LoRA) & 61.39 & \textbf{22.00} & \textbf{73.10}\\
OPT-IML-MAX-30B (PEMA w/o rct) & \textbf{70.29}& 23.38 & 51.24 \\
\midrule
GYAFC (Entertainment \& Music)& \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{FormImp}  \\
\midrule
OPT-IML-MAX-30B (LoRA) & 59.76 & \textbf{23.97}& \textbf{68.29}\\
OPT-IML-MAX-30B (PEMA w/o rct) & \textbf{64.82}& 26.32 & 42.61\\
\bottomrule

==> tbls/data_statistic.tex <==
Dataset                        & \multicolumn{1}{c}{Train}     & \multicolumn{1}{c}{Valid}            & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Length of $\mathcal{E}$}\\
\midrule
GYAFC (F\&R) & \multicolumn{1}{r}{51,967} &\multicolumn{1}{r}{2,788}& \multicolumn{1}{r}{1,332}       & \multicolumn{1}{r}{691,531}     \\
GYAFC (E\&M)  & \multicolumn{1}{r}{52,595} &\multicolumn{1}{r}{2,877}& \multicolumn{1}{r}{1,416}       & \multicolumn{1}{r}{695,465}      \\
WMT22  & \multicolumn{1}{r}{388,482} & \multicolumn{1}{r}{2,203} & \multicolumn{1}{r}{1,984}       & \multicolumn{1}{r}{20,983,482}     \\
%GSM8k  & \multicolumn{1}{r}{6,800} & \multicolumn{1}{r}{673} & \multicolumn{1}{r}{1,319}       & \multicolumn{1}{r}{647,619}     \\
\bottomrule

==> tbls/hyperparameter.tex <==
\sys    & \multicolumn{1}{c}{} \\
\midrule
Random seed                 & 123          \\
Number of rank                        & 512 or 8        \\
Batch size                  & 40,960       \\
Adam $lr$                     & 1e-03     \\
Adam $(\beta_1, \beta_2)$                  & (0.9, 0.999) \\
Adam $eps$                    & 1e-08     \\
\midrule
\multicolumn{1}{l}{LoRA}    & \multicolumn{1}{c}{} \\
\midrule
Random seed                 & 123          \\
Number of rank                       & 512 or 8        \\
Batch size                  & 10 to 30      \\
Adam $lr$                     & 1e-03     \\
Adam $(\beta_1, \beta_2)$                  & (0.9, 0.999) \\
Adam $eps$                    & 1e-08     \\
LoRA $\alpha$                       & 1            \\
Merge weight                & FALSE        \\
\midrule
\multicolumn{1}{l}{$k$NN-LM}    & \multicolumn{1}{c}{} \\
\midrule
Random seed                 & 1            \\
Number of centroids learn   & 4,096         \\
Quantized vector size       & 64           \\
Number of clusters to query & 32           \\
Distance function           & L2 Distance  \\
\bottomrule

==> tbls/informal_mitigation.tex <==
Percentage        & \multicolumn{1}{c}{Original Informal} & \multicolumn{1}{c}{Reference Formal} & \multicolumn{2}{c}{OPT-IML-MAX-30B} & \multicolumn{2}{c}{with $k$NN-LM} & \multicolumn{2}{c}{with \sys} \\
\midrule
Family \& Relationships \\
\midrule
Slang Abbreviation         & 525       & 307.75      &352          & 32.95\%            &350         & 33.33\%           &\textbf{305}         & \textbf{41.90\%}        \\
All Capital                & 68        & 0           &61           & 10.29\%            &61          & 10.29\%           &\textbf{4}           & \textbf{94.12\%}        \\
Redundant Word             & 39        & 2           &\textbf{1}   & \textbf{97.44\%}   &\textbf{1}  & \textbf{97.44\%}  &4                    & 89.74\%                 \\
Non-Capital Start          & 636       & 1.5         &2            & 99.69\%            &2           & 99.69\%           &\textbf{0}           &\textbf{100.00\%}        \\
\midrule
Entertainment \& Music \\
\midrule
Slang Abbreviation         & 651       & 485.75      &548          & 15.82\%                 &538         & 17.36\%              &\textbf{482} & \textbf{25.96\%}       \\
All Capital                & 36        & 0           &32           & 11.11\%                 &34          & 5.56\%               &\textbf{6}   & \textbf{83.33\%}      \\
Redundant Word             & 49        & 17.75       &\textbf{5}   & \textbf{89.80\%}        &\textbf{5}  & \textbf{89.80\%}     &8            & 83.67\%       \\
Non-Capital Start          & 655       & 7           &2            & 99.69\%                 &2           & 99.69\%              &\textbf{0}   & \textbf{100.00\%}       \\
\bottomrule

==> tbls/model_comparison_full.tex <==
&&\multicolumn{4}{l}{WMT22 (EN$\rightarrow$DE)}                                                                                                                                                               & \multicolumn{4}{|l}{GSM8k}                                                                                               \\
Model                  & \multicolumn{1}{c|}{\# Trainable} & \multicolumn{1}{c}{}         & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{}      & \multicolumn{1}{c|}{}                  & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}                  \\
                       & \multicolumn{1}{c|}{Parameters}   & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET}     & \multicolumn{1}{c}{-}                 & \multicolumn{1}{|c}{Accuracy} & \multicolumn{1}{c}{Not Answered} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}                 \\
\midrule
OPT-IML-MAX-1.3B           &                                  & 9.55                             & 19.13                                 & 57.24                          &                                       & 1.74                          & 25.68                        &                           &                                       \\
OPT-IML-MAX-1.3B (FT)      &                                  & 10.15                             & \underline{17.23}                                 & 61.44                          &                                       & 1.36                          & 1.14                        &                           &                                       \\
OPT-IML-MAX-1.3B (FT-top2) &                                  & 3.57                             & 25.64                                 & 38.35                          &                                       & \textbf{2.50}                          & 0.30                        &                           &                                       \\
%OPT-IML-MAX-1.3B (Adapter) &                                  &                              &                                  &                           &                                       &                           &                         &                           &                                       \\
OPT-IML-MAX-1.3B (kNN-LM)  &                                  & 8.07                             & 60.50                                 & 41.75                          &                                       & 1.82                          & 20.53                        &                           &                                       \\
OPT-IML-MAX-1.3B (LoRA${}_{r=8}$)  &                                  & 3.25                             & 25.63                                 & 40.50                          &                                       & 1.89                          & 20.00                        &                           &                                       \\
OPT-IML-MAX-1.3B (LoRA${}_{r=512}$)  &                                  & 4.28                             & 24.97                                 & 39.32                          &                                       & 2.12                          & 19.09                        &                           &                                       \\
OPT-IML-MAX-1.3B (PEMA${}_{r=8}$)    &                                  & \underline{11.75}                             & 21.43                                 & \underline{61.50}                          &                                       & 1.59                          & 22.12                        &                           &                                       \\
OPT-IML-MAX-1.3B (PEMA${}_{r=512}$)    &                                  & \textbf{12.87}                            & \textbf{18.52}                                 & \textbf{64.16}                          &                                       & \underline{2.20}                          & 22.88                        &                           &                                       \\
\midrule
LLAMA-7B           &                                  & 2.78                            & 36.40                                 &  39.49                          &                                       & \textbf{6.36}                          & 0.08                        &                           &                                       \\
%LLAMA-7B (Adapter) &                                  &                              &                                  &                           &                                       &                           &                         &                           &                                       \\
LLAMA-7B (kNN-LM) &                                  & 0.07                             & 35.12                                 & 38.53                          &                                       & 3.11                          & 0.98                        &                           &                                       \\
LLAMA-7B (LoRA${}_{r=8}$)  &                                  & 10.92                             & \underline{12.84}                                 & 66.88                          &                                       & 3.56                          & 0.00                        &                           &                                       \\
LLAMA-7B (LoRA${}_{r=512}$)  &                                  & \underline{11.46}                             & 12.91                                 & \underline{67.48}                          &                                       & 3.64                          & 0.00                        &                           &                                       \\
LLAMA-7B (PEMA${}_{r=8}$)    &                                  & 3.88                             & \textbf{4.74}                                  & 48.44                          &                                       & \underline{6.06}                          & 0.53                        &                           &                                       \\
LLAMA-7B (PEMA${}_{r=512}$)    &                                  & \textbf{14.50}                             &  19.89                                 & \textbf{70.31}                          &                                       & 3.56                          & 1.82                        &                           &                                       \\
\midrule
OPT-IML-MAX-30B           &                                  & 18.22                             & 22.15                                 & 77.41                          &                                       & 0.68                          & 78.71                        &                           &                                       \\
%OPT-IML-MAX-30B (Adapter) &                                  &                              &                                  &                           &                                       &                           &                         &                           &                                       \\
OPT-IML-MAX-30B (kNN-LM) &                                  & 16.65                             & 46.11                                 & 62.98                          &                                       & 0.76                          & 35.91                        &                           &                                       \\
OPT-IML-MAX-30B (LoRA${}_{r=8}$)  &                                  & 16.05                             & 23.77                                 & 74.01                          &                                       & 0.38                          & 78.33                        &                           &                                       \\
OPT-IML-MAX-30B (LoRA${}_{r=512}$)  &                                  & 8.26                             & \textbf{10.63}                                 & 69.41                          &                                       & 0.30                          & 79.02                        &                           &                                       \\
OPT-IML-MAX-30B (PEMA${}_{r=8}$)    &                                  & \underline{18.33}
                             & 26.98                                 & \underline{77.75}                          &                                       & \textbf{3.03}                          & 16.21                        &                           &                                       \\
OPT-IML-MAX-30B (PEMA${}_{r=512}$)    &                                  & \textbf{19.22}                             & \underline{21.85}                                 & \textbf{79.21}                          &                                       & \underline{1.89}                          & 45.99                        &                           &                                       \\
\midrule
&&\multicolumn{4}{l}{GYAFC (Family \& Relatationships)}                                                                                                                                           & \multicolumn{4}{|l}{GYAFC (Entertainment \& Music)}                                                                      \\
Model                  & \multicolumn{1}{c|}{\# Trainable} & \multicolumn{1}{c}{}         & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{}      & \multicolumn{1}{c|}{Formality}         & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{Formality}         \\
                       & \multicolumn{1}{c|}{Parameters}   & \multicolumn{1}{c}{sBLEU}    & \multicolumn{1}{c}{PPL}          & \multicolumn{1}{c}{COMET} & \multicolumn{1}{c}{Increasement (\%)} & \multicolumn{1}{|c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} & \multicolumn{1}{c}{Increasement (\%)} \\
\midrule
OPT-IML-MAX-1.3B           &                                  & 55.00                             & 26.96                                 & 81.67                          & 11.05                                      & 53.98                         & 35.27                        & 81.79                          & 10.67                                      \\
OPT-IML-MAX-1.3B (FT)      &                                  & 29.17                             & \underline{19.83}                                 & \underline{84.06}                          & \underline{52.28}                                      & 31.50                          & \underline{26.20}                        & \underline{83.52}                          & \underline{46.82}                                      \\
OPT-IML-MAX-1.3B (FT-top2) &                                  & 21.60                             & 21.41                                 & \textbf{84.26}                          & \textbf{59.00}                                      & 23.94                          & 28.55                        & \textbf{83.73}                          & \textbf{51.52}                                      \\
%OPT-IML-MAX-1.3B (Adapter) &                                  &                              &                                  &                           &                                       &                           &                         &                           &                                       \\
OPT-IML-MAX-1.3B (kNN-LM)  &                                  & \underline{56.69}                             & 36.54                                 & 81.50                          & 16.26                                      & \underline{54.74}                          & 48.00                        & 81.13                          & 14.46                                      \\
OPT-IML-MAX-1.3B (LoRA${}_{r=8}$)  &                                  & 23.13                             & 23.89                                 & 76.26                          & 45.68                                      & 18.41                          & 26.36                        & 74.40                          & 46.00                                      \\
OPT-IML-MAX-1.3B (LoRA${}_{r=512}$)  &                                  & 20.98                             & 23.71                                & 75.24                          & 45.71                                      & 15.57                          & \textbf{24.90}                        & 72.92                          & 46.32                                      \\
OPT-IML-MAX-1.3B (PEMA${}_{r=8}$)    &                                  & 56.29                             & 30.22                                 & 80.79                          & 36.27                                      & 54.22                          & 40.27                        & 80.70                          & 35.52                                      \\
OPT-IML-MAX-1.3B (PEMA${}_{r=512}$)    &                                  & \textbf{64.82}                             & \textbf{19.52}                                 & 80.63                          & 41.90                                      & \textbf{61.24}                          & 27.89                        & 81.74                          & 36.28                                      \\
\midrule
LLAMA-7B           &                                  & 20.18                             & \underline{11.43}                                 & 37.42                          & 42.81                                      & 24.14                          & 18.02                        & 56.65                          & 44.81                                      \\
%LLAMA-7B (Adapter) &                                  &                              &                                  &                           &                                       &                           &                         &                           &                                       \\
LLAMA-7B (kNN-LM) &                                  & 1.72                            & \textbf{9.36}                                 & 44.85                          & 55.13                                      & 1.94                          & \textbf{10.90}                        & 45.56                          & 68.61                                      \\
LLAMA-7B (LoRA${}_{r=8}$)  &                                  & 14.80                             & 12.39                                 & 72.38                          & \textbf{88.43}                                      & 12.69                          & \underline{16.18}                        & 71.56                          & \textbf{89.70}                                      \\
LLAMA-7B (LoRA${}_{r=512}$)  &                                  & \underline{52.67}                             & 19.86                                 & \textbf{82.65}                          & 72.23                                      & \underline{52.15}                          & 25.21                        & \textbf{82.41}                          & \underline{71.28}                                      \\
LLAMA-7B (PEMA${}_{r=8}$)    &                                  & 48.88                             & 17.26                                 & \underline{73.59}                          & \underline{80.21}                                      & 45.73                          & 22.89                        & 72.17                          & 70.85                                      \\
LLAMA-7B (PEMA${}_{r=512}$)    &                                  & \textbf{63.99}                             & 17.21                                 & 38.05                          & 61.40                                      & \textbf{60.88}                          & 22.06                        & \underline{81.32}                          & 60.94                                      \\
\midrule
OPT-IML-MAX-30B           &                                  & 60.41                             & 22.82                                 & 82.23                          & 29.33                                      & 57.60                          & 30.53                        & 81.79                          & 23.88                                      \\
%OPT-IML-MAX-30B (Adapter) &                                  &                              &                                  &                           &                                       &                           &                         &                           &                                       \\
OPT-IML-MAX-30B (kNN-LM) &                                  & 61.02                             & 31.55                                 & 82.86                          & 29.80                                      & 58.58                          & 42.80                        & 82.54                          & 23.39                                      \\
OPT-IML-MAX-30B (LoRA${}_{r=8}$)  &                                  & 61.28                             & \underline{22.21}                                 & \textbf{84.50}                          & 73.33                                      & 59.48                          & \underline{23.84}                        & \underline{83.38}                          & \textbf{68.35}                                      \\
OPT-IML-MAX-30B (LoRA${}_{r=512}$)  &                                  & 61.39                             & 23.71                                 & \underline{84.49}                          & 73.10                                      & 59.76                          & \textbf{20.50}                        & \textbf{83.47}                          & \underline{68.29}                                      \\
OPT-IML-MAX-30B (PEMA${}_{r=8}$)    &                                  & \underline{62.87}                             & 27.36                                 & 82.84                          & 46.05                                      & \underline{60.12}                          & 37.23                        & 82.42                          & 38.92                                      \\
OPT-IML-MAX-30B (PEMA${}_{r=512}$)    &                                  & \textbf{70.84}                             & \textbf{18.16}                                 & 83.54                          & 52.35                                      & \textbf{65.43}                          & 25.03                        & 82.57                          & 44.63                                      \\
\bottomrule

==> tbls/model_comparison_gsm8k.tex <==
Model                 && \multicolumn{1}{|c|}{\# Trainable} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Not Answered} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
                      && \multicolumn{1}{|c|}{Parameters}   &                           &                         &       &\\

\midrule
OPT-IML-1.3B           && &      1.74\%&             25.68\%&             &                   \\
OPT-IML-1.3B (FT)      && & soon           &                    &             &                   \\
OPT-IML-1.3B (FT-top2) && & soon           &                    &             &                   \\
OPT-IML-1.3B (Adapter) && &            &                    &             &                   \\
OPT-IML-1.3B (KNN)     && & soon           &                    &             &                   \\
OPT-IML-1.3B (LoRA)    && & soon           &                    &             &                   \\
OPT-IML-1.3B (AdaLoRA) && &            &                    &             &                   \\
OPT-IML-1.3B (\sys)    && &      2.20\%&             22.88\%&             &                   \\
\midrule
LLaMA-7B               && &      6.36\%&              0.08\%&             &                   \\
LLaMA-7B (Adapter)     && &            &                    &             &                   \\
LLaMA-7B (KNN)         && & soon           &                    &             &                   \\
LLaMA-7B (LoRA)        && &            &                    &             &                   \\
LLaMA-7B (AdaLoRA)     && &            &                    &             &                   \\
LLaMA-7B (\sys)        && &      3.56\%&              1.82\%&             &                   \\
\midrule
OPT-IML-30B            && &      0.68\%&             78.71\%&             &                   \\
OPT-IML-30B (Adapter)  && &            &                    &             &                   \\
OPT-IML-30B (KNN)      && & soon           &                    &             &                   \\
OPT-IML-30B (LoRA)     && & soon           &                    &             &                   \\
OPT-IML-30B (AdaLoRA)  && &            &                    &             &                   \\
OPT-IML-30B (\sys)     && &      1.89\%&             45.99\%&             &                  \\
\bottomrule


==> tbls/model_comparison_gyafc.tex <==
Model                 && \multicolumn{1}{|c|}{\# Trainable} & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} & \multicolumn{1}{c}{FI (\%)} \\
                      && \multicolumn{1}{|c|}{Parameters}   &                           &                         &       &\\

\midrule
Family \& Relationships \\
\midrule
OPT-IML-1.3B          && 0& 55.00      & 26.96             & 81.67       & 11.05             \\
OPT-IML-1.3B (FT)     && 1,315,758,080& soon           &                    &             &                   \\
OPT-IML-1.3B (FT-top2)&& & soon           &                    &             &                   \\
OPT-IML-1.3B (Adapter)&& &            &                    &             &                   \\
OPT-IML-1.3B (KNN)    && & soon           &                    &             &                   \\
OPT-IML-1.3B (LoRA)   && 2,359,296& 56.68      & 30.36              & 80.22       & 25.99            \\
OPT-IML-1.3B (AdaLoRA)&& &            &                    &             &                   \\
OPT-IML-1.3B (\sys)   && 2,097,152& 64.82      & 19.52              & 80.63       & 41.90             \\
\midrule
LLaMA-7B          && & 20.18      & 11.43              & 37.42       & 42.81             \\
LLaMA-7B (Adapter)&& &            &                    &             &                   \\
LLaMA-7B (KNN)    && & soon           &                    &             &                   \\
LLaMA-7B (LoRA)   && &            &                    &             &                   \\
LLaMA-7B (AdaLoRA)&& &            &                    &             &                   \\
LLaMA-7B (\sys)   && & 63.99      & 17.21              & 38.05       & 61.40             \\
\midrule
OPT-IML-30B            && & 60.14                     & 33.49                              & 83.12      & 27.86                   \\
OPT-IML-30B (Adapter)  && &            &                    &             &                   \\
OPT-IML-30B (KNN)      && & 61.55                     & 33.62                              & 83.40      & 29.61                   \\
OPT-IML-30B (LoRA)     && & 61.77                     & 29.93                              & 83.48      &  31.44                  \\
OPT-IML-30B (AdaLoRA)  && &            &                    &             &                   \\
OPT-IML-30B (\sys)     && & \textbf{70.98}           & \textbf{26.42}                   & \textbf{83.52}            & \textbf{51.85}                  \\
\midrule
Entertainment \& Music \\
\midrule
OPT-IML-1.3B          && & 53.98      & 35.27              & 81.79       & 10.67             \\
OPT-IML-1.3B (FT)     && & soon           &                    &             &                   \\
OPT-IML-1.3B (FT-top2)&& & soon           &                    &             &                   \\
OPT-IML-1.3B (Adapter)&& &            &                    &             &                   \\
OPT-IML-1.3B (KNN)    && & soon           &                    &             &                   \\
OPT-IML-1.3B (LoRA)   && & 44.48      & 10.39              & 81.91       & 78.83             \\
OPT-IML-1.3B (AdaLoRA)&& &            &                    &             &                   \\
OPT-IML-1.3B (\sys)   && & 61.24      & 27.89              & 81.74       & 36.28             \\
\midrule
LLaMA-7B          && & 24.14      & 18.02              & 56.65       & 44.81             \\
LLaMA-7B (Adapter)&& &            &                    &             &                   \\
LLaMA-7B (KNN)    && & soon           &                    &             &                   \\
LLaMA-7B (LoRA)   && &            &                    &             &                   \\
LLaMA-7B (AdaLoRA)&& &            &                    &             &                   \\
LLaMA-7B (\sys)   && & 60.88      & 22.06              & 81.32       & 60.94             \\
\midrule
OPT-IML-30B            && &  57.26                    &  45.11                  & 82.54              &  23.61          \\
OPT-IML-30B (Adapter)  && &            &                    &             &                   \\
OPT-IML-30B (KNN)      && &  58.00                    &  44.85                  & 81.02              &  22.47          \\
OPT-IML-30B (LoRA)     && &  59.43                    &  37.78                  & \textbf{83.36}     & 29.32           \\
OPT-IML-30B (AdaLoRA)  && &            &                    &             &                   \\
OPT-IML-30B+\sys       && &  \textbf{67.01}           & \textbf{35.97}          & 82.86              & \textbf{46.74}  \\
\bottomrule


==> tbls/model_comparison_rank.tex <==
Model & \multicolumn{3}{c}{WMT22 (EN$\rightarrow$DE)} & \multicolumn{3}{c}{GYAFC (Family \& Relationships)} & \multicolumn{3}{c}{GYAFC (Entertainment \& Music)}\\
& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{} & \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{} \\
& \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{FormImp} & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{FormImp} \\
\midrule
OPT-IML-MAX-1.3B (LoRA${}_{r=8}$) & 3.25& 66.16 & 40.50 & 23.13 & \textbf{18.82} & {\underline{45.68}} & 18.41 & {\textbf{19.68}} & {\underline{46.00}} \\
OPT-IML-MAX-1.3B (LoRA${}_{r=512}$) & 4.28& 61.25& 39.32 & 20.98 & {\underline{19.07}} & \textbf{45.71}& 15.57 & \underline{19.71}& \textbf{46.32}\\
OPT-IML-MAX-1.3B (PEMA${}_{r=8}$) & {\underline{11.75}} & {\underline{44.73}} & {\underline{61.50}} & {\underline{56.29}} & 21.41 & 36.27 & {\underline{54.22}} & 23.42 & 35.52 \\
OPT-IML-MAX-1.3B (PEMA${}_{r=512}$) & \textbf{12.87}& \textbf{42.62}& \textbf{64.16}& \textbf{64.82}& 23.15& 41.90 & \textbf{61.24}& 24.28 & 36.28 \\
\midrule
LLaMA-7B (LoRA${}_{r=8}$) & 10.92 & 52.01 & 66.88 & 14.80 & \textbf{17.85}& \textbf{88.43}& 12.69 & \textbf{19.66} & \textbf{89.70}\\
LLaMA-7B (LoRA${}_{r=512}$) & {\underline{11.46}} & \underline{51.36} & {\underline{67.48}} & {\underline{52.67}} & \underline{22.42} & 72.23 & \underline{52.15} & \underline{24.74} & {\underline{71.28}} \\
LLaMA-7B (PEMA${}_{r=8}$) & 3.88& \textbf{45.48} & 48.44 & 48.88 & 26.69 & {\underline{80.21}} & 45.73 & 32.03 & 70.85 \\
LLaMA-7B (PEMA${}_{r=512}$) & \textbf{14.50}& 54.26 & \textbf{70.31}& \textbf{63.99}& 23.19 & 61.40 & \textbf{60.88} & 26.00 & 60.94 \\
\midrule
OPT-IML-MAX-30B (LoRA${}_{r=8}$)& 16.05 & 47.66 & 74.01 & 61.28 & {\underline{21.99}} & \textbf{73.33}& 59.48 & {\underline{24.01}} & \textbf{68.35}\\
OPT-IML-MAX-30B (LoRA${}_{r=512}$)& 16.03& \underline{46.97}& 74.65 & 61.39 & 22.00 & {\underline{73.10}} & 59.76 & \textbf{23.97}& {\underline{68.29}} \\
OPT-IML-MAX-30B (PEMA${}_{r=8}$)& {\underline{18.33}} & 47.40 & {\underline{77.75}} & {\underline{62.87}} & \textbf{21.75} & 46.05 & {\underline{60.12}} & 24.10 & 38.92 \\
OPT-IML-MAX-30B (PEMA${}_{r=512}$)& \textbf{19.22}& {\textbf{46.62}} & \textbf{79.21}& \textbf{70.84}& 22.04& 52.35 & \textbf{65.43}& 25.53 & 44.63\\
\bottomrule

==> tbls/model_comparison_wmt22.tex <==
Model                 && \multicolumn{1}{|c|}{\# Trainable} & \multicolumn{1}{c}{sBLEU} & \multicolumn{1}{c}{PPL} & \multicolumn{1}{c}{COMET} & \multicolumn{1}{c}{-} \\
                      && \multicolumn{1}{|c|}{Parameters}   &                           &                         &       &\\

\midrule
OPT-IML-1.3B          && & 9.55       & 19.13              & 57.24       &                   \\
OPT-IML-1.3B (FT)     && & 10.15      & 16.31              & 61.44       &                   \\
OPT-IML-1.3B (FT-top2)&& & soon           &                    &             &                   \\
OPT-IML-1.3B (Adapter)&& &            &                    &             &                   \\
OPT-IML-1.3B (KNN)    && & soon           &                    &             &                   \\
OPT-IML-1.3B (LoRA)   && & 10.90      & 20.04              & 60.47       &                   \\
OPT-IML-1.3B (AdaLoRA)&& &            &                    &             &                   \\
OPT-IML-1.3B (\sys)   && & 12.87      & 18.52              & 64.16       &                   \\
\midrule
LLaMA-7B          && & 0.00       & 36.40              & 39.49       &                   \\
LLaMA-7B (Adapter)&& &            &                    &             &                   \\
LLaMA-7B (KNN)    && & soon           &                    &             &                   \\
LLaMA-7B (LoRA)   && &            &                    &             &                   \\
LLaMA-7B (AdaLoRA)&& &            &                    &             &                   \\
LLaMA-7B (\sys)   && & 14.50      & 19.89              & 70.31       &                   \\
\midrule
OPT-IML-30B            && & 18.22      & 22.15              & 77.41       &                   \\
OPT-IML-30B (Adapter)  && &            &                    &             &                   \\
OPT-IML-30B (KNN)      && & soon           &                    &             &                   \\
OPT-IML-30B (LoRA)     && & soon           &                    &             &                   \\
OPT-IML-30B (AdaLoRA)  && &            &                    &             &                   \\
OPT-IML-30B (\sys)     && & 19.22      & 21.85              & 79.21       &                  \\
\bottomrule


==> tbls/prompt_examples.tex <==
Task  & Instruction                                                     \\
\midrule
WMT22 & Translate this from English to German:                          \\
      & [English Input]                                                 \\
      & German: [Generated Output]                                      \\
\midrule
GYAFC & Convert the following informal sentence into a formal sentence: \\
      & Informal: [Informal Input]                                      \\
      & Formal: [Generated Output]                                      \\
%\midrule
%GSM8K & Problem: [Math Question Input]                                  \\
%      & Solution: [Generated Solution]                                 \\
\bottomrule
